MoPro: Webly Supervised Learning with Momentum Prototypes

We propose a webly-supervised representation learning method that does not suffer from the annotation unscalability of supervised learning, nor the computation unscalability of self-supervised learning. Most existing works on webly-supervised representation learning adopt a vanilla supervised learning method without accounting for the prevalent noise in the training data, whereas most prior methods in learning with label noise are less effective for real-world large-scale noisy data. We propose momentum prototypes (MoPro), a simple contrastive learning method that achieves online label noise correction, out-of-distribution sample removal, and representation learning. MoPro achieves state-of-the-art performance on WebVision, a weakly-labeled noisy dataset. MoPro also shows superior performance when the pretrained model is transferred to down-stream image classification and detection tasks. It outperforms the ImageNet supervised pretrained model by +10.5 on 1-shot classification on VOC, and outperforms the best self-supervised pretrained model by +17.3 when finetuned on 1\% of ImageNet labeled samples. Furthermore, MoPro is more robust to distribution shifts. Code and pretrained models are available at https://github.com/salesforce/MoPro.

==> table/fig_voc.tex <==
\begin{wrapfigure}{r}{0.45\textwidth}
	\centering
	\includegraphics[trim=0 0 0 1cm,width=0.44\textwidth]{VOC_1shot}
	\caption{Write some caption here}
	
	\label{fig:voc}
\end{wrapfigure}

==> table/tbl_dg.tex <==
\begin{table*}[t!]
	\centering	
	\begin{tabular}	{l l  |  c c c c | c}
		\toprule
		\multirow{2}{*}{Method}  & \multirow{2}{*}{Pretrain dataset}& \multicolumn{4}{c}{target domain} & \\
		& &  photo  & artpainting & cartoon & sketch & Avg. \\
		\midrule
		
		CE & ImageNet & 98.3&82.5 &74.6 &74.3 &82.4\\
		%wCE & WebVision &  & & &\\
		MoPro& WebVision &  & & & &\\		
		\bottomrule
	\end{tabular}
\caption
{
\small	
\textbf{Domain generalization}.
}
\label{tbl:dg}	
\end{table*}			

==> table/tbl_imagenet.tex <==
\begin{table*}[t!]
	\centering	
	\begin{tabular}	{l l l |  c c}
		\toprule
		Method & Pretrain dataset&  &Top-1 & Top-5 \\
		\midrule
		
		CE & ImageNet & \multirow{3}{*}{linear classifier}& & \\
		wCE & WebVision &  & & \\
		MoPro& WebVision &  & & \\
		\midrule
		CE & ImageNet &end-to-end &76.2 & \\
		\midrule
		CE & WebVision &  \multirow{2}{*}{finetuning}& & \\
		MoPro& WebVision &  &77.9 &94.0 \\				
		\bottomrule
	\end{tabular}
\caption
{
\small	
\textbf{ImageNet classification}.
}
\label{tbl:imagenet}	
\end{table*}			

%\begin{table*}[t!]
%	\centering	
%	\begin{tabular}	{l l |  c c| c c}
%		\toprule
%		\multirow{2}{*}{Method} & \multirow{2}{*}{Pretrain dataset}&  \multicolumn{2}{c|}{Linear classifier}& \multicolumn{2}{c}{End-to-end}\\
%		& & 	 Top-1 & Top-5&Top-1 & Top-5 \\
%		\midrule
%		
%		CE & ImageNet &  75.2 & 92.4 &76.2 & \\
%		CE & WebVision-V1.0 & 72.6& 90.8 & & \\
%		MoPro& WebVision-V1.0   & 75.0&92.3 & &\\
%		
%		\bottomrule
%	\end{tabular}
%	\caption
%	{
%		\small	
%		\textbf{ImageNet classification}.
%	}
%	\label{tbl:imagenet}	
%\end{table*}		
